MovieNet: A Holistic Dataset for Movie Understanding

Recent years have seen remarkable advances in visual understanding. However, how to understand a story-based long video with artistic styles, e.g. movie, remains challenging. In this paper, we introduce MovieNet -- a holistic dataset for movie understanding. MovieNet contains 1,100 movies with a large amount of multi-modal data, e.g. trailers, photos, plot descriptions, etc. Besides, different aspects of manual annotations are provided in MovieNet, including 1.1M characters with bounding boxes and identities, 42K scene boundaries, 2.5K aligned description sentences, 65K tags of place and action, and 92K tags of cinematic style. To the best of our knowledge, MovieNet is the largest dataset with richest annotations for comprehensive movie understanding. Based on MovieNet, we set up several benchmarks for movie understanding from different angles. Extensive experiments are executed on these benchmarks to show the immeasurable value of MovieNet and the gap of current approaches towards comprehensive movie understanding. We believe that such a holistic dataset would promote the researches on story-based long video understanding and beyond. MovieNet will be published in compliance with regulations at https://movienet.github.io.

==> articles/conclusion.tex <==
% !TEX root = ../main.tex

\section{Appendix}
\label{sec:appendix}

(1) samples of different kinds of annotations
(2) Annotation Tools
(3) Compare MovieNet to domain specific datasets

\subsection{Person Identity Annotation}
two stage of annotation

\subsection{Synopsis Alignment}
We collected the associations following the procedure below.
(1) We provide the annotators with a complete overview of each movie, including the character list, reviews, etc., to ensure they are familiar with the
movies.
(2) We carry out the annotation procedure in two stages, from coarse to fine. At the first stage, each movie is divided into $64$ clips, each lasting for around $2$ minutes. For each synopsis paragraph, an annotator is asked to select a segment, \ie a subsequence of N consecutive clips, that cover the corresponding description. At the second stage, annotators adjust the temporal boundaries of the resultant segments to make them better aligned with the paragraphs. This two-stage procedure leads to a collection of paragraph-segment pairs.
(3) We dispatch each paragraph to three annotators and only retain those annotations with high consistency among them. Here, the consistency is measured in
terms of temporal IoU among the annotations. 
